Factor-augmented tree ensembles

This manuscript proposes to extend the information set of time-series regression trees with latent stationary factors extracted via state-space methods. In doing so, this approach generalises time-series regression trees on two dimensions. First, it allows to handle predictors that exhibit measurement error, non-stationary trends, seasonality and/or irregularities such as missing observations. Second, it gives a transparent way for using domain-specific theory to inform time-series regression trees. Empirically, ensembles of these factor-augmented trees provide a reliable approach for macro-finance problems. This article highlights it focussing on the lead-lag effect between equity volatility and the business cycle in the United States.

==> ch2_annex/subsect1.tex <==
\begin{definition}[Sample size]
	Denote with $n$, $T$ and $p$ three finite natural numbers.
\end{definition}

\begin{assumption}[Target data]
	Let $\vect{Y}$ be a $T \times 1$ vector of observations for the time periods $t=1, \ldots, T$ representing a finite realisation of the real-valued and mean-stationary stochastic process $\{Y_{t} : t \in \mathbb{Z}\}$. 
\end{assumption}

\begin{assumption}[Predictors: standard regression trees]
	Let $\vect{Z}$ be a $n \times T$ matrix of observations for the time periods $t=1, \ldots, T$ representing a finite realisation of the real-valued and mean-stationary stochastic process $\{\vect{Z}_{t} = (Z_{1,t} \; \ldots \; Z_{n,t})' : t \in \mathbb{Z}\}$. Furthermore, let $\vect{X}_t \defeq (Y_t \; Z_{1,t} \; \ldots \; Z_{n,t})'$ be $m \times 1$ dimensional, with $m \defeq 1+n$.
\end{assumption}

\begin{remark}
	Throughout the manuscript, the dependency on $n, T$ and $p$ is highlighted only when strictly necessary to ease the reading experience. Furthermore, specific realisations at some integer point in time $t$ and their general value in the underlying stochastic processes are denoted with the same symbols. However, it should be clear from the context whether the manuscript is referring to the first or second category.
\end{remark}

This article describes the regression trees as non-linear forecasting models for $Y_t$ based on the information included in $\vect{X}_{t-1}, \ldots,  \vect{X}_{t-p}$. These methodologies are jointly determined by a directed graph and a regression model. In order to describe the model itself in more detail, it is necessary to introduce first a series of graph-theoretical definitions.

\begin{definition}[Binary trees] \label{def:trees}
	A binary tree is a directed acyclic graph with vertices and edges denoted with $\mathscr{V}$ and $\mathscr{E}(\mathscr{V})$ respectively, and the following four properties:
	\begin{enumerate2}
		\item $\mathscr{V} \subset \mathbb{N}$, $|\mathscr{V}| \geq 1$ and $\mathscr{E}(\mathscr{V}) \subseteq \{(v,w) : (v,w) \in \mathscr{V}^2,\, v<w\}$;
		\item $\mathscr{V}_1$ denotes the so-called root node (or, vertex) and $\indeg(\mathscr{V}_1) = 0$;
		\item for every $v \in \mathscr{V}$, the $\outdeg(v) \in \{0,2\}$; 
		\item there exists a unique walk from the root node $\mathscr{V}_1$ to any other vertex in $\mathscr{V}$.
	\end{enumerate2}
\end{definition}

\begin{remark}
	Three interesting points follow from \cref{def:trees}. First, all binary tree edges are unidirectional and point away from the root node $\mathscr{V}_1$. Second, in binary trees with order $|\mathscr{V}| > 1$, the size $|\mathscr{E}(\mathscr{V})| > 0$ and even. Third, if the size is larger than zero, the first element of the pair $\mathscr{E}_{i}(\mathscr{V})$ is placed at the same position in $\mathscr{E}_{i+1}(\mathscr{V})$, but not in any other edge, for every odd integer $1 \leq i < |\mathscr{E}(\mathscr{V})|$.
\end{remark}

\Crefrange{def:leaves}{def:labels} provide further structure to the binary tree. The mathematical concepts herein defined are helpful to formalise the forecasting model. 

\begin{definition}[Leaves] \label{def:leaves}
	Define a binary tree leaf as a vertex with zero outer degrees. Hence, let $\mathscr{F}(\mathscr{V}) \defeq \{v : v \in \mathscr{V},\, \outdeg(v)=0\}$ be the set of leaves in the binary tree. The complement for this set is $\bar{\mathscr{F}}(\mathscr{V}) \defeq \{v : v \in \mathscr{V},\, \outdeg(v) \neq 0\}$.
\end{definition}

\begin{definition}[Root to leaf walk] \label{def:walks}
	For every $v \in \mathscr{F}(\mathscr{V})$, define $\mathscr{W}_v (\mathscr{V}) \subseteq \mathscr{E}(\mathscr{V})$ as the set of edges representing the walk from the root node to the vertex $v$.
\end{definition}

\begin{definition}[Labels] \label{def:labels}
	Label every $v \in \bar{\mathscr{F}}(\mathscr{V})$ with a triplet $\vect{c}_v \equiv \vect{c}_v (m, p)$ such that $c_{1,v} \in \{1, \ldots, m\}$, $c_{2,v} \in \{1, \ldots, p\}$ and $c_{3,v} \in \mathbb{R}$.
\end{definition}

\input{./ch2_annex/example_tree}

\begin{example}[Simple binary tree] \label{example:binary}
	This example describes \crefrange{def:trees}{def:labels} on the basis of the binary tree reported in \cref{fig:tree}. Starting from the most basic items, this graph has seven vertices and six edges. Following \cref{def:trees}, $\mathscr{V} = \{1,2,\ldots,7\}$, and $\mathscr{E}(\mathscr{V}) = \{(1,2),\, (1,3),\, (2,4),\, (2,5),\, (5,6),\, (5,7)\}$. The vertices can be categorised and divided into two disjoint sets depending on whether they have a outer degree different from zero. This is achieved by using the set of leaves $\mathscr{F}(\mathscr{V}) = \{3, 4, 6, 7\}$ and its complement $\bar{\mathscr{F}}(\mathscr{V}) = \{1, 2, 5\}$. The sets of edges representing the walks from the root node to each leaf are $\mathscr{W}_3 (\mathscr{V}) = \{(1,3)\}$, $\mathscr{W}_4 (\mathscr{V}) = \{(1, 2),\, (2, 4)\}$, $\mathscr{W}_6 (\mathscr{V}) = \{(1, 2),\, (2, 5),\, (5, 6)\}$ and $\mathscr{W}_7 (\mathscr{V}) = \{(1, 2),\, (2, 5),\, (5, 7)\}$. Examples of vertex labels are reported in \cref{fig:tree}.
\end{example}

\begin{assumption}[Directed graphs]
	Following common practise in the literature, the regression trees are built around the graph structure introduced in \cref{def:trees} and further specified in \crefrange{def:leaves}{def:labels}.
\end{assumption}

The forecasting model implied by a regression tree is formalised in \crefrange{assumption:model}{assumption:condexp}. This gives a generalised additive model \citep{hastie1987generalized} compatible with complex data dynamics.

\begin{assumption}[Regression tree model]
	Assume that
	\begin{align*}
		Y_t = \sum_{u \in \mathscr{F}(\mathscr{V})} b_u \prod_{(v,w) \in \mathscr{W}_u (\mathscr{V})} f(\vect{X}_{t-1}, \ldots, \vect{X}_{t-p}, \vect{c}_{v}, w) + \epsilon_t,
	\end{align*}
	
	\noindent where every $b_u$ is a finite real scalar,
	\begin{align*}
		&f(\vect{X}_{t-1}, \ldots, \vect{X}_{t-p}, \vect{c}_{v}, w) = \begin{cases}
			1 & \text{if } X_{c_{1,v},\, t-c_{2,v}} \geq c_{3,v} \text{ and } w \text{ is even}, \\
			1 & \text{if } X_{c_{1,v},\, t-c_{2,v}} < c_{3,v} \text{ and } w \text{ is odd}, \\
			0 & \text{otherwise},
		\end{cases}
	\end{align*}
	
	\noindent $\epsilon_t \widesim{i.i.d.} \left(0, \sigma^2\right)$ and for any integer $t$. For simplicity, the parameters are also denoted as
	\begin{align*}
		\vect{\theta} \defeq \begin{pmatrix}
			\vect{b} \\ 
			\vect{c}_1 \\ 
			\vdots \\ 
			\sigma
		\end{pmatrix}.
	\end{align*}
\end{assumption}

\begin{assumption}[Conditional expectation of the innovation] \label{assumption:condexp}
	Assume that
	\begin{align*}
		\expect(\epsilon_t | \vect{X}_{t-s}) = \expect(\epsilon_t | \vect{X}_{t-1}, \ldots, \vect{X}_{t-p}) = \expect(\epsilon_t | \vect{X}_{t-1}, \ldots, \vect{X}_{t-p}, \vect{\theta}, \mathscr{V}) = 0,
	\end{align*}
	
	\noindent for any integer $t$, $s < t$, valid $\vect{\theta}$ and $\mathscr{V}$.
\end{assumption}

\begin{example}[Simple regression tree]
	This example shows the interconnections between binary and regression trees, building on \cref{example:binary}. Assume, for the sake of this example, that $p=2$, $T=3$ and
	\begin{align*}
		\vect{X} = \begin{pmatrix}
			5 & 4.5 & 6 \\
			12 & 10 & 11 \\
			0.5 & 2.0 & 1.5
		\end{pmatrix}.
	\end{align*}
	
	\noindent Recall that for the graph in \cref{fig:tree} $\mathscr{W}_3 (\mathscr{V}) = \{(1,3)\}$, $\mathscr{W}_4 (\mathscr{V}) = \{(1, 2),\, (2, 4)\}$, $\mathscr{W}_6 (\mathscr{V}) = \{(1, 2),\, (2, 5),\, (5, 6)\}$ and $\mathscr{W}_7 (\mathscr{V}) = \{(1, 2),\, (2, 5),\, (5, 7)\}$. Hence, at $t=T$, the products described in \cref{assumption:model} evaluated at each leaf are
	\begin{align*}
		&\prod_{(v,w) \in \mathscr{W}_3 (\mathscr{V})} f(\vect{X}_{2}, \vect{X}_{1}, \vect{c}_{v}, w) = \indicator_{X_{3,1} < 1.5} = 1, \\
		&\prod_{(v,w) \in \mathscr{W}_4 (\mathscr{V})} f(\vect{X}_{2}, \vect{X}_{1}, \vect{c}_{v}, w) = \indicator_{X_{3,1} \geq 1.5}\;\indicator_{X_{2,2} \geq 10} = 0, \\
		&\prod_{(v,w) \in \mathscr{W}_6 (\mathscr{V})} f(\vect{X}_{2}, \vect{X}_{1}, \vect{c}_{v}, w) = \indicator_{X_{3,1} \geq 1.5}\;\indicator_{X_{2,2} < 10}\;\indicator_{X_{1,2} \geq 5} = 0, \\
		&\prod_{(v,w) \in \mathscr{W}_7 (\mathscr{V})} f(\vect{X}_{2}, \vect{X}_{1}, \vect{c}_{v}, w) = \indicator_{X_{3,1} \geq 1.5}\;\indicator_{X_{2,2} < 10}\;\indicator_{X_{1,2} < 5} = 0.
	\end{align*}
	
	\noindent Thus,
	\begin{align*}
		Y_3 = b_3 + \epsilon_t,
	\end{align*}
	
	\noindent for some finite real scalar $b_3$.
\end{example}

Regression trees are estimated under \crefrange{assumption:model}{assumption:lags}. Without loss of generality, this manuscript focusses on the one-step ahead forecast in \cref{def:forecast} only. Long-run predictions can be generated by computing direct forecasts \citep[e.g., following, in spirit, the approach in ][]{marcellino2006comparison}. 

\begin{assumption}[Lags] \label{assumption:lags}
	Assume that the number of lags $0 < p \ll T-1$.
\end{assumption}

\begin{definition}[One-step ahead forecast]\label{def:forecast} Let $\vect{\hat{\theta}}_s\,(\vect{\gamma})$ and $\hat{\mathscr{V}}_s$ denote the parameters and vertices estimated on the information set available at time $1 \leq s \leq T$. Under \crefrange{assumption:model}{assumption:lags}, the forecast for $Y_{t+1}$, conditional on this structure is
	\begin{align*}
		\hat{Y}_{t+1, s}(\vect{\gamma}) \defeq \sum_{u \in \mathscr{F}(\hat{\mathscr{V}_s)}} \hat{b}_{u,s} \prod_{(v,w) \in \mathscr{W}_u (\hat{\mathscr{V}_s)}} f(\vect{X}_{t}, \ldots, \vect{X}_{t-p+1}, \vect{\hat{c}}_{v,s}, w),
	\end{align*}
	
	\noindent where $\vect{\gamma}$ is a vector of hyperparameters, for every integer $p \leq t \leq T$ and $1 \leq s \leq T$.
\end{definition}

\noindent This article estimates the model using the CART algorithm: an iterative method that builds the tree recursively partitioning the data in \crefrange{assumption:data_target}{assumption:data_predictors} over the predictor space. The details for the algorithm are described in \cite{breiman1984classification} and this manuscript uses \href{https://github.com/bensadeghi/DecisionTree.jl}{DecisionTree.jl} to implement it.
